Evaluation of Siamese Networks for Semantic Code Search

With the increase in the number of open repositories and discussion forums, the use of natural language for semantic code search has become increasingly common. The accuracy of the results returned by such systems, however, can be low due to 1) limited shared vocabulary between code and user query and 2) inadequate semantic understanding of user query and its relation to code syntax. Siamese networks are well suited to learning such joint relations between data, but have not been explored in the context of code search. In this work, we evaluate Siamese networks for this task by exploring multiple extraction network architectures. These networks independently process code and text descriptions before passing them to a Siamese network to learn embeddings in a common space. We experiment on two different datasets and discover that Siamese networks can act as strong regularizers on networks that extract rich information from code and text, which in turn helps achieve impressive performance on code search beating previous baselines on $2$ programming languages. We also analyze the embedding space of these networks and provide directions to fully leverage the power of Siamese networks for semantic code search.

==> 6_discussion.tex <==


% This hints at the possibility that the narrow funnel in the network caused by having $2$ output units at the top of the Siamese network act as a regualizer that force the lower layers to learn more meaningful embeddings which in turn helps the overall task when using those embeddings for retrieval.

% We now focus on just the DCS layer. To understand the superior performance of $S_{emb}=2$, we visualize the embeddings learnt by the DCS-Siamese network at the DCS layer for two architectures with $S_{emb}=200$ and $S_{emb}=2$ respectively as shown in Figure \ref{fig:SembComparison}. We consider the SQL dataset for visualization since the raw queries and code snippets are not available for the Java dataset. We use tSNE to plot the DCS embeddings for $S_{emb}=200$. A quick examination reveals that the embedding space has sharp, distinct clusters when $S_{emb}=2$, whereas the clusters when $S_{emb}=200$ are relatively diffused. Further, we manually examined some of the clusters and evaluated the questions that are mapped to those clusters. Some samples are listed in Table \ref{tab:clusternames}. Apart from the fact that the clusters in the right figure are smaller for the four sets of queries we examined, the ones on the left blend in with the other points in the figure, implying that the network has done a poor job at learning to distinguish between different queries at the DCS layer when $S_{emb}=2$. Its is unsurprising that we achieve better MRR when Code retrieval is performed at the DCS layer for $S_{emb}=2$. We analyze this effect due to $S_{emb}$ further in the next section.

\section{Discussion}
In this section, we analyze the results obtained above to understand the behavior of the DCS-Siamese network. We focus on this architecture since it outperforms all other architectures and baseline models considered. Specifically, we would like to analyze three observations:

\textit{A. Regularization effect of the DCS-Siamese model over the original DCS architecture}

We visualize the embeddings learnt by the DCS network \cite{DCS} and the output of the DCS extraction network, after using the Siamese network, for the text descriptions in the StaQC SQL dataset using t-SNE \cite{maaten2008visualizing} in Figure \ref{fig:SembComparison}. We consider the SQL dataset for visualization since the raw queries and code snippets are not available for the Java dataset. 

A quick examination reveals that the embedding space has sharp, distinct clusters for the DCS-Siamese network (right), whereas the clusters in the original DCS network (left) are relatively smaller and more scattered. Further, we manually examined some of the clusters and evaluated the questions that are mapped to those clusters. Few samples are listed in Table \ref{tab:clusternames}. For the query groups \textit{DATE} and \textit{JOIN}, the clusters are scattered in different regions for the original DCS network. Also, the cluster corresponding to the \textit{MAX} query group is adjacent to the \textit{DATE} cluster. Comparatively, for the same query groups, the clusters for the DCS-Siamese network are well separated and coherent. This highlights the role of Siamese network as a regularizer when applied on top of the DCS network. The Siamese network seemingly helps in rearranging the embedding space leading to more meaningful representations, bringing similar inputs (in this case, texts) closer in the embedding space. This effect is further reflected in the better retrieval MRR of the DCS-Siamese network. 

% We observe this result for both the datasets. In our experiments, the difference between the results of $S_{emb}=2$ and $S_{emb}=200$ variesd but we observe a clear trend in favor of $S_{emb}=2$. To understand the superior performance of $S_{emb}=2$, we visualize the embeddings learnt by the DCS-Siamese network at the DCS layer for two architectures with $S_{emb}=200$ and $S_{emb}=2$ respectively as shown in Figure \ref{fig:SembComparison}. We consider the SQL dataset for visualization since the raw queries and code snippets are not available for the Java dataset. We use tSNE to plot the DCS embeddings for $S_{emb}=200$. A quick examination reveals that the embedding space has sharp, distinct clusters when $S_{emb}=2$, whereas the clusters when $S_{emb}=200$ are relatively diffused. Further, we manually examined some of the clusters and evaluated the questions that are mapped to those clusters. Some samples are listed in Table \ref{tab:clusternames}. Apart from the fact that the clusters in the right figure are smaller for the four sets of queries we examined, the ones on the left blend in with the other points in the figure, implying that the network has done a poor job at learning to distinguish between different queries at the DCS layer when $S_{emb}=2$. Its is unsurprising that we achieve better MRR when Code retrieval is performed at the DCS layer for $S_{emb}=2$.

% This hints at the possibility that the narrow funnel in the network caused by having $2$ output units at the top of the Siamese network act as a regualarizer that forces the lower layers to learn more meaningful embeddings, which in turn helps the overall task when using those embeddings for retrieval. We did observe 1 exception to this when we evaluated on the Siamese layer output with $S_{emb}=200$. However, the difference in performance was only marginal. This visualization, coupled with the results in Table \ref{tab:ourresults} clearly establishes the value of the $S_{emb}=2$ DCS-Siamese network. 

% We have also observed the inverse of this regularization effect for other values of $S_{emb}$ and the model performance gradually degrades as the value of $S_{emb}$ increases.


% This also explains why the clusters corresponding to a given set of similar queries are extremely well defined for the embeddings at the DCS layer than the embeddings at the top layer of the network. The restriction to compact information into 2 dimensions has led to a loss of information in the 2-d embedding space for a given set of queries, but this has led the DCS layer to learn a rich set of embeddings.

% \textbf{figure out how to show and pitch the scatter plot of the correct-wrong pairs of points, if at all needed}

% If this argument indeed holds, we would see a gradual loss of information as we look at the embeddings at the other intermediate layers of the network, upto the final layer. We visualize the embeddings of the layer between the DCS output and the final layer using tSNE for the same set of queries in table X. Indeed, we see that the cluster representing the queries in the embedding space of the intermediate layer is somewhat scattered, but not as much as that of the final layer.

\begin{table}[]
\small
\centering
\begin{tabular}{|p{0.2\columnwidth}|p{0.7\columnwidth}|}
\hline
\textbf{Type} & \textbf{Sample Questions} \\
\hline
\multirow{5}{*}{SORTING} & How should I use order by on distinct entities? \\
 & Sort numbers after letters in order by \\
 & SQL query to produce results in reverse order \\
 & How to add condition in order by?\\
 & Sort result based on parent child connection in SQL \\
 \hline
\multirow{5}{*}{DELETE} & How to delete with a join and no id? \\
 & Delete a database record along with its latest records \\
 & SQL delete duplicate rows with lowest number \\
 & Sysntax to remove record when build subset from other tables \\
 & Delete record based on text found in field \\
 \hline
\end{tabular}
\caption{Sample questions related to Sorting and Deletion queries.}
\label{tab:example-questions}
\end{table}

\textit{B. For the DCS-Siamese network, retrieval on the output of DCS layer achieves higher MRR}

We now focus on the actual embeddings learnt at the different layers of the DCS-Siamese network with $S_{emb}=2$.  Figure \ref{fig:emb_tsneplots_semb2} shows the embedding plots of the final Siamese layer (left) and the output of the DCS layer (right). We focus on two specific set of queries shown in Table \ref{tab:example-questions}. We believe having $2$ output units results in a much stronger regularization effect leading to these two sets of questions being mapped to well-defined regions in the embedding space. 
% As discussed earlier, the regularization effect of having $2$ output units results in much better embedding at the DCS layer resulting in these $2$ sets of questions being mapped to well-defined regions in the embedding space. 
However, due to the low dimensionality at the final layer, there is a tremendous loss of information that deprives the layer of any meaning to its representations. The purpose of the representations is to simply reduce the loss function and guide the gradient forcing the lower layers to learn a much more meaningful embedding. The actual meaning to representations of code and text is hence obtained at a lower layer.

This effect is also consistent for embeddings of code, as observed in Figure \ref{fig:code_tsneplots_semb2}, where we generated 
 a plot of the embeddings of the SQL queries corresponding to the questions in Table \ref{tab:example-questions}. In comparison, to the DCS layer embedding of the DSC-Siamese network (right side of Figure \ref{fig:emb_tsneplots_semb2}), we observed more than one clusters for the \textit{sorting questions} (red circles in Figure \ref{fig:code_tsneplots_semb2}). 
 
  This is due to the fact that any question that involves a deletion would more-or-less be always translated to a 'DELETE FROM' clause in code (blue squares). However, there could be several questions that might not explicitly ask about sorting, but still require sorting as an intermediate step in the answer. The code corresponding to such answers would have an 'ORDER BY' clause, but depending on the actual question, might involve other SQL clauses.

To summarize, $S_{emb}=2$ has a far stronger regularizing effect on the network as compared to larger values. However, due to this effect, there seems to be a loss of information in the final layers of the Siamese network and hence, the embeddings learned by the lower layers of the network contain richer information for the Code retrieval task.

\textit{C. The DCS extraction network greatly outperforms the other extraction networks when combined with Siamese networks}

We selected the DCS setup as an extraction network because it leveraged a variety of features from code. Although we believe these features are collectively responsible for the impressive performance of the DCS-Siamese model, when considered individually with a Siamese network, they are unable to provide enough information during training, leading to an extremely poor model. This hints at the possibility that providing code as input to a deep learning network may not be straightforward and although the DCS features worked well, there are possibly other features that need to be discovered. Also, some code features might be useful for certain datasets, but not for all.


% \textbf{once you hav explained select and find/get/fetch are far apart, give a solution how to fix that}
% This result is surprising since [togther we stand paper] has reported impressive results using siamese networks with simple preprocessing and a conv-pooling-relu-FC network. However, when applied to code retrieval, siamese networks with different model architectures and embeddings sizes do not perform as well as other models such as [dcs][coacor] that rely on extracting multiple features from code. We hypothesize that this is due to different vocabularies as well as different mearnings of the same terms in code and text. For instance, the question and answer pairs of [together we stanbd paper] come from the same language (barring technical terms in the answers), even though the distributions of these terms in questions and answers might be different.

% \textbf{actually, we need to think more on this and come up with more convincing experiemnts and results}



% Using an ablation study, we identify that API sequence tokens provide the highest performance of all the features used by the DCS model \textbf{also mention this in training/model details of the simple models}. 

==> 7_conclusion.tex <==
\section{Conclusion and Future Work}
Siamese networks can achieve impressive performance on Code Retrieval tasks by learning a meaningful embedding of code and it's description text. This performance is heavily reliant on an appropriate representation of code and we have observed that the DCS architecture can achieve this reasonably well. However, while we have some understanding of the regularization provided by the Siamese network, we would like to study this effect in more detail as future work. We would also like to validate our observations on more datasets and other tasks involving code and natural language text such as Code Summarization and Code Synthesis.

==> backup_content.tex <==
\section{Introduction}
\begin{itemize}
  \item Motivating Code Search
  \item What and Why (importance)
  \item Usecase and samples
  \item Introduce Siamese
  \item Introduce the questions we will try to answer in the paper
\end{itemize}
The rest of the paper is organized as follows - blah blah

Searching for code fragments is a very common activity in software development. The advent of large code repositories like GitHub\footnote{https://github.com/} and StackOverflow\footnote{https://stackoverflow.com/} has only increased the number of developers to rely on these repositories to search and reuse existing code \citeZipInputStream zipIn = new ZipInputStream(new FileInputStream(zipFilePath));
        ZipEntry entry = zipIn.getNextEntry();
{reiss2009semantics}. Given its reliance and significance there are still primarily two challenges with the code retrieval system that hinders developers from successful code search a)Difference in the vocabulary of code and search text b)Lack of semantic understanding of search text.

Traditional Information systems does not work well for code search tasks, as there is often little shared vocabulary between the source code and the search texts. Often times, you will find developers who are new to a particular programming language searching for code snippets in a context free natural language manner. The choice of words used to search may not correspond or overlap with the code snippets leading to failure of these traditional information retrieval systems. 
Example : Developer has a functional requirement to check for expected condition to during the runtime to be implemented using java programming language. A seasoned java programmer might be aware of \textit{java assert} keyword, thereby resulting in a relevant code snippet which satisfies the requirement. A naive java developer who is not familiar with the programming language might make a query from the requirement  \textit{java check condition correctness} which does not result in relevant code snippet.

Other times, lack of deeper understanding of the search query leads to inconsistent and irrelevant code snippets. Example \textit{refactor code with multiple arguments in java} has relevant java terms but if the search engine cannot understand the developer is trying to look for snippets that can refactor method or constructor which usually takes arguments cannot suggest snippets that use Builder Pattern or  grouping logical objects as relevant answers. In such cases, though there is certain overlap in keywords, there is a need for deeper understanding of the input query to retrieve the relevant snippet.

Usage of deep neural models have shown significant improvements in many tasks including language tasks \textbf{cite papers}. This success can be largely attributed for its capability to represent the text better as vectors and their ability to learn complex patterns automatically for the given task without much supervision.
One such model that is hugely popular for determining similarity between text documents is siamese neural networks\cite{bromley1994signature}\textbf{more citations}. First introduced by \cite{bromley1994signature} a \textbf{explain better siamese} siamese network consists of two or more sub networks that share the same weights. They can work in tandem on different input vectors produce comparable output vectors. This has been successfully applied in many similarity tasks in image domain \textbf{citations}. Since code is also a text data and code retrieval can be seen as a similarity tasks where in the distance between semantically relevant code snippet and search text tend to be closer. We apply siamese model for this code search task.

We observe that applying siamese network does not yield desired results. Then, we took DCS \textbf{cite} considered as state of the art model for this task and stacked siamese network on top. Interestingly, we find that this combined network beats the benchmark results across multiple data sources. We study this behavior  further and attempt to reason with a series of experiments which are captured in the following sections.



% \tikz \draw[] (0,0) rectangle (\linewidth, -1in) node[pos=.2]{Answer Here:};


